Intuitionistic Euler-Venn Diagrams (extended)

We present an intuitionistic interpretation of Euler-Venn diagrams with respect to Heyting algebras. In contrast to classical Euler-Venn diagrams, we treat shaded and missing zones differently, to have diagrammatic representations of conjunction, disjunction and intuitionistic implication. We present a cut-free sequent calculus for this language, and prove it to be sound and complete. Furthermore, we show that the rules of cut, weakening and contraction are admissible.

==> discussion.tex <==

\section{Discussion}
\label{sec:disc}
In this section, we compare our calculus  with existing proof systems for Euler diagrams 
and discuss its properties, implications and possible extensions. 


Burton et al. analysed %typical 
strategies for completeness proofs
of diagrammatic languages \cite{Burton2012}. 
%Their main result is that 
%in languages with lower expressivity like Euler diagrams, Spider diagrams
%and Constraint Diagrams, 
They emphasise that usually the strategy 
 how to prove an Euler diagram \(E\) from the assumptions \(D_1, \dots, D_n\) is to first  create  a maximal
\setlength\intextsep{0pt}
\begin{wrapfigure}{l}{.48\textwidth}
    \begin{tikzpicture}
      \node (diag1) {
        \begin{tikzpicture}[euler]
          \node[fill=white,contour, minimum size = 1.15cm] (cnode) {};
          \node[fill=white,contour, minimum size = .4cm] (b1node) at (cnode) {}; 
            \node[xshift=-.75cm] at (cnode) {\(c\)};
            \node[xshift=-.35cm] at (b1node) {\(b\)};
        \end{tikzpicture}      
      };
      \node[right =-.15cm of diag1] (and) {\(\land\)};
      \node[right =-.15cm of and] (a) {\((a \implies b)\)};      
      \node[right =-.15cm of a] (impl2) {\(\implies\)};
      \node[right =-.150cm of impl2] (diag1) {
        \begin{tikzpicture}[euler]
            \node[fill=white,contour, minimum size = 1.15cm] (anode) {};
            \node[fill=white,contour, minimum size = .4cm, xshift =-.25cm] (bnode) at (anode) {}; 
            \node[xshift=-.95cm] at (anode) {\(c\)};
            \node[xshift=-.55cm] at (bnode) {\(a\)};
        \end{tikzpicture}
      };
      
    \end{tikzpicture}
  \caption{Heterogeneous Euler Diagrams }
  \label{fig:hetero-prop-diag}
\end{wrapfigure}
 diagram \(D_{\mathit{max}}\) 
incorporating the information from all of the \(D_i\). Then, all information
that is not part of \(E\) will be removed from \(D_{\mathit{max}}\). 
%For our sequent calculus however,
We do not apply this strategy. Instead, 
%almost
%all 
the rules % we employ in the completeness proof 
decompose the diagrams, with
the only exception being the rules to introduce missing zones. This % misalignment
is due to the similarity of our calculus to typical sentential calculi. % \slcomment{DISCUSSION of PROOF SYSTEMS from DIAGRAMS 2010!!}

The proof system presented in this paper is related to both systems presented
by Mineshima et al. \cite{Mineshima2010}. It is oriented towards refutations, like
the resolution calculus for Venn-diagrams, but also contains rules for the connectives
and diagrammatic elements, like natural deduction for Euler diagrams. However, our
language comprises both Venn-diagrams and Euler diagrams without shading.

\setlength{\intextsep}{\savedintextsep}

% We only used the rules \(\mzDecL\) and \(\mzDecR\) to reduce the number of
% contours in the diagrams to achieve completeness in diagrams
% already equivalent to \(\top\). However, these rules 
% may serve within a proof to reduce the clutter \cite{John2005,Alqadah2014} in the diagrams, 
% and thus possibly enhance the readability of the proof.

We can extend our calculus to facilitate heterogeneous sequents in a rather simple
way. We can allow compound diagrams to be mixed with propositional 
% \setlength\intextsep{0pt}
% \begin{wrapfigure}{l}{.24\textwidth}
%    \(\sequent{\leftSeq, a}{\rightSeq, \unitaryLiteral{a}{.2cm}}\)\\[.5em]
% \(   \sequent{\leftSeq, \unitaryLiteral{a}{.2cm}}{\rightSeq, a}\)  
% \caption{Het. Axioms}
%  \label{fig:hetero-prop-ax}
% \end{wrapfigure}
% \setlength{\intextsep}{\savedintextsep}
formulas, as for example shown in Fig.~\ref{fig:hetero-prop-diag}. The rules for Boolean
operators can then be directly applied to propositional formulas. The only
extension we need to incorporate into the calculus are heterogeneous axioms. % (see Fig.~\ref{fig:hetero-prop-ax}).
 \begin{align*}
   \sequent{\leftSeq, a}{\rightSeq, \unitaryLiteral{a}{.2cm}} &&   \sequent{\leftSeq, \unitaryLiteral{a}{.2cm}}{\rightSeq, a}  
 \end{align*}
% \setlength\intextsep{0pt}
% \begin{wrapfigure}{l}{.2\textwidth}
%   \begin{tabular}{l}    
% \(\sequent{\leftSeq, a}{\rightSeq, \unitaryLiteral{a}{.2cm}}\)\\[1em]
% \(\sequent{\leftSeq, \unitaryLiteral{a}{.2cm}}{\rightSeq, a}\)
%   \end{tabular}
% \caption{Het. Axioms}
% \label{fig:het-axioms}
% \end{wrapfigure}
% \setlength{\intextsep}{\savedintextsep}
This system then allows us to reason about heterogeneous Euler diagrams. However, it is hardly
a heterogeneous \emph{reasoning} system in the sense of Barwise and Etchemendy \cite{Barwise1996},
since it does not include rules to transfer information from one representation into the other.

Furthermore, it is simple to amend our calculus to represent
intuitionistic logic instead of classical propositional logic. To that end,
we restrict the succedent of sequents to be a single formula, and change 
the Boolean rules accordingly\footnote{Compare with the textbook by Negri et al. \cite{Negri2001}}. 
For most of
the diagrammatic rules, this change is sufficient as well, the only exceptions are
\(\singDecL\) and \(\singDecR\). However, we can change these rules as follows.
\begin{center}
  \begin{tabular}{c}    
    \prftree[r]{\(\scriptstyle \singDecL^I\)}
    {\sequent{\leftSeq, d}{ \unitaryLiteral{n_1}{.15cm}}}
    {\dots}
    {\sequent{\leftSeq,d }{ \unitaryLiteral{n_k}{.15cm}}}
    {\sequent{\leftSeq, \unitaryLiteral{o_1}{.15cm}}{D}}
    {\dots}
    {\sequent{\leftSeq, \unitaryLiteral{o_l}{.15cm}}{D}}
    {\sequent{\leftSeq, d}{D}}
    \\[1em]
    \prftree[r]{\(\scriptstyle \singDecR^I\)}
    {\sequent{\leftSeq, \unitaryLiteral{n_1}{.15cm}, \dots, \unitaryLiteral{n_k}{.15cm}}{ \unitaryLiteral{o_i}{.15cm}}}
    {\sequent{\leftSeq}{d}}
  \end{tabular}
\end{center}
That is, in \(\singDecL^I\), we keep the %original
 diagram in the antecedent for
the branches with the new literals in the succedent, while we omit it in the branches, where
we add literals to the antecedent. For \(\singDecR^I\), we choose a single occurrence 
of a literal to keep in the succedent. These changes are similar to the changes for
the Boolean operators. Observe that the semantics presented in Sect.~\ref{sec:euler}
is no longer suited for this proof system. We would have 
to define a semantics based on intuitionistic models, for example Heyting algebras.
However, how such a semantics should look like is not obvious.
It would be interesting to study the connection of
this proof system to traditional proof systems for Euler diagrams, since 
the graphical notations for intuitionistic logic are sparse. Notable
exceptions are the work of de Freitas and Viana \cite{deFreitas2012}, defining
a graphical calculus for relational reasoning, and Alves et al. \cite{Alves2011}, in
which they present a visualisation of intuitionistic proofs. 
In a similar way, we could try to change the system to reflect substructural logics, i.e.,
logics for which the structural rules of weakening, contraction and/or permutation do 
not hold\footnote{More precisely, these
logics are typically \emph{defined} by the lack of these rules.}. 
 However, in these logics, new operators arise %in addition to the typical Boolean ones,
and  would have to be reflected in the diagrams as well. Such a radical change
is not part of this paper, and left as future work.
Of course, classical diagrammatic systems are possible ways to extend our calculus 
as well. A natural next step is an extension to treat Spider diagrams or
Constraint diagrams.  

A sequent calculus style proof system is suited for automatic proof search. Hence,
an implementation into the theorem prover Speedith \cite{Urbas2015} is obvious future
work, since it already supports
backward reasoning and several proof branches. Furthermore, 
extending the tactics within Speedith \cite{Linker2017}
to our calculus would allow us to  delay the application of rules creating new branches
in the proof.  


% \begin{itemize}
% %\item comparison with completeness results (Jim et al. in Euler Workshop): Instead of creating
% %maximal diagram (like Shin, etc), we directly decompose diagrams ==> proof construction
% %more straightforward
% % \item Even though decomposition on contours not needed for completeness (true??), we can use 
% % them to decrease clutter and complexity of diagrams (reference to clutter studies)
% \item comparison with purely sentential system: difference in breadth/width of proof tree (concrete
% elements of unitary diagrams/how specific the information inside a single shaded zone is)
% % \item heterogeneous reasoning system immediate: add axioms where one side is a literal, the other a proposition
% %   \begin{itemize}
% %   \item however, the ``reasoning'' part is still not really heterogeneous. No rules to infer 
% % formula from diagram and vice versa. Only connection at the leaves of deductions.
% %   \end{itemize}
% % \item restrict the right hand side of sequents to single diagrams gives us intuitionistic euler diagrams? we need
% % to change decompositional rules however (and make use of negative literals). Does removing the classical
% % semantics impact the other/traditional E/V proof systems? 
% \end{itemize}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "int-dia-sequent"
%%% End: 


==> venn.tex <==
\section{Venn Diagrams}
\label{sec:venn}
A Venn diagram consists of a set of \emph{contours}, dividing
the space enclosed by a 
% \setlength\intextsep{0pt}
% \begin{wrapfigure}{l}{.16\textwidth}
%   \begin{tikzpicture}[euler]
%     \node[fill=lightgray,contour, minimum size = 1.15cm] (cnode) {};
%     \node[fill=white,contour, minimum size = .4cm] (b1node) at (cnode) {}; 
%     \node[xshift=-.75cm] at (cnode) {\(c\)};
%     \node[xshift=-.35cm] at (b1node) {\(b\)};
%   \end{tikzpicture}
% \caption{Euler diagram}
% \label{fig:euler}
% \end{wrapfigure}
% \setlength{\intextsep}{\savedintextsep}
bounding rectangle into all possible different zones. A zone
may be shaded.
%(see Fig.~\ref{fig:euler} 
%for
%an example). 
Traditionally, each contour represents a set, and the diagram
restricts the possible relations between these sets. 
To keep the connection with intuitionistic logic as defined in the
previous section\slcomment{Add section on intuitionistic syntax and semantics}, we
slightly alter the semantics. That is, instead of an arbitrary set,
a contour represents an \emph{open set} in the topology of
an intuitionistic model.


      % \begin{definition}[Zone]
%\label{def:zone}
A \emph{zone} for a finite set of contours \(\contours \subset \vars\) is a tuple
\((\zin, \zout)\), where \(\zin\) and \(\zout\) are disjoint 
subsets of \(\contours\) such that \(\zin \cup \zout = \contours\).
The set of all zones for a given set of contours is denoted
by \(\vennzones{\contours}\).
%\end{definition}

\begin{definition}[Abstract Syntax]
  \label{def:euler-syntax}
  A \emph{unitary} Venn diagram is a tuple \(d = (\contours, \ezones)\),
where \(\ezones\) are a set of zones for  for \(\contours\), the  \emph{shaded zones} 
 of \(d\). 
% For a unitary diagram \(d\), we will also refer to the set of its
% \emph{missing zones} \(\mzones{d} = \vennzones{\contours} \setminus \zones\).
The syntax of  Venn diagrams is then given as
 \begin{align*}
   D &::= d \mid   D \land D \mid D \lor D \mid 
 D \implies D \, ,
 \end{align*}
where \(d\) is
% a
 unitary.
%Euler 
%diagram. 
%The other Boolean
%connectives are given by the usual abbreviations, e.g.,
%\(D_1 \lor D_2 \equiv \lnot (\lnot D_1 \land \lnot D_2)\) and \(D_1 \implies D_2 \equiv \lnot D_1 \lor D_2\).
%We will call 
Venn diagrams of the form  \(D_1 \land D_2\), \(D_1 \lor D_2\)
and
 \(D_1 \implies D_2\)  are \emph{compound}.
\end{definition}

%Note that 
We allow for the %special 
diagrams \(\top = (\emptyset, \emptyset)\)
and \(\bot = (\emptyset,  \{(\emptyset, \emptyset)\})\).
\setlength\intextsep{0pt}
\begin{wrapfigure}[4]{l}{.22\textwidth}
%\begin{center}
\centering
%\subfloat[]{
\unitaryLiteral{a}{.5cm}
%  \label{fig:literal-unitary-pos}
%}
%\subfloat[]{
\unitaryLiteralNeg{a}{.5cm}
%  \label{fig:literal-unitary-neg}
%}
%\end{center}
\caption{Literals}
  \label{fig:literal-unitary}
\end{wrapfigure}
\setlength{\intextsep}{\savedintextsep}
% With this % naming
%convention, 
Similarly to sentential intuitionistic logic, we define negation by \(\lnot D \equiv D \implies \bot\). A \emph{literal} is a unitary diagram for a single contour, with exactly one
shaded zone.
%Unitary diagrams
%\(d\) for a single contour \(c\), in which exactly one zone is shaded, are called \emph{literals}. 
If the zone \((\emptyset, \{c\})\) is shaded in a literal, then we call it \emph{positive}, otherwise
it is \emph{negative} (see Fig.~\ref{fig:literal-unitary}). Observe that our notion of literals slightly deviates
from the original definition of Stapleton and Masthoff \cite{Stapleton2007}.


\begin{definition}[Zone Semantics]
  Given an intuitionistic model \(\model = (\universe, \topo)\), a \emph{valuation} is a function \(\valSing \colon \vars \to \topo\), assigning an open set to each variable.
We denote the set of all valuations by \(\vals\).
Let \(z=(\zin, \zout)\) be a zone.
% and \(\valSing \colon \vars \to \bool\) be a valuation.
 The  
\emph{semantics} of \(z\) is an open set  of \(\topo\), given
by
 \begin{align*}
   \zsem{z}{\model}{\valSing} & = \interior{\bigcap_{c \in \zin} \val{c}{}  \cap \bigcap_{c \in \zout} \comp{\val{c}{}}}
 \end{align*}
\end{definition}

We distinguish between two types of semantics for unitary diagrams. The \emph{positive} semantics
consists of the union of the visualised, non-shaded zones. That is, the diagram
denotes, which parts of the topology are actually represented. The \emph{negative} semantics, however,
determines, which parts of the topology are missing. Hence, the negative semantics
are given by first computing the union of the zone semantics, and then taking the interior of the
complement of this union.


\begin{definition}[Positive Semantics]
  The positive semantics of Venn diagrams is
 defined by
 \begin{align*}
   \psem{d}{\model}{\valSing} & = \bigcup_{z \in \vennzones{\contours} \setminus \ezones} \zsem{z}{\model}{\valSing} \\
   \psem{D_1 \land D_2}{\model}{\valSing} & = \psem{D_1}{\model}{\valSing} \cap \psem{D_2}{\model}{\valSing} \\
   \psem{D_1 \implies D_2}{\model}{\valSing} & = \interior{\comp{\psem{D_1}{\model}{\valSing}} \cup \psem{D_2}{\model}{\valSing}}  \\
   \psem{D_1 \lor D_2}{\model}{\valSing} & = \psem{D_1}{\model}{\valSing} \cup \psem{D_2}{\model}{\valSing}
%  \sem{\lnot D} & = \vals \setminus \sem{D} &
 \end{align*}
%\(  \sem{d}  = \bigcup_{z \in \zones \setminus \ezones} \sem{z} \) and
%\( \sem{D_1 \implies D_2} = (\vals \setminus \sem{D_1}) \cup \sem{D_2} \),
where \(d\) is unitary and  \(D_1\), \(D_2\) are arbitrary 
Venn diagrams. If \(\psem{D}{\model}{\valSing} = \universe\), for all intuitionistic models \(\model\)
and valuations \(\val\) then we call \(D\) \emph{positively valid}, denoted
by \(\models_P D\). Otherwise, \(D\) is \emph{positively falsifiable}. Furthermore, let
\(\mathcal{D}\) be a set of Venn diagrams. We say that \(D\) is a \emph{consequence}
of \(\mathcal{D}\), if, and only if, \(\left( \bigcap_{ D^\prime \in \mathcal{D}} \psem{D^\prime}{\model}{\valSing}\right) \subseteq \psem{D}{\model}{\valSing}\) for all models \(\model\) and valuations \(\valSing\).  
\end{definition}

\begin{definition}[Negative Semantics]
  The negative semantics of Venn diagrams is
 defined by
 \begin{align*}
   \nsem{d}{\model}{\valSing} & = \interior{\comp{\bigcup_{z \in \ezones} \zsem{z}{\model}{\valSing}}} \\
   \nsem{D_1 \land D_2}{\model}{\valSing} & = \nsem{D_1}{\model}{\valSing} \cap \nsem{D_2}{\model}{\valSing} \\
   \nsem{D_1 \implies D_2}{\model}{\valSing} & = \interior{\comp{\nsem{D_1}{\model}{\valSing}} \cup \nsem{D_2}{\model}{\valSing}}  \\
   \nsem{D_1 \lor D_2}{\model}{\valSing} & = \nsem{D_1}{\model}{\valSing} \cup \nsem{D_2}{\model}{\valSing}
%  \sem{\lnot D} & = \vals \setminus \sem{D} &
 \end{align*}
%\(  \sem{d}  = \bigcup_{z \in \zones \setminus \ezones} \sem{z} \) and
%\( \sem{D_1 \implies D_2} = (\vals \setminus \sem{D_1}) \cup \sem{D_2} \),
where \(d\) is unitary and  \(D_1\), \(D_2\) are arbitrary 
Venn diagrams. If \(\nsem{D}{\model}{\valSing} = \universe\), for all intuitionistic models \(\model\)
and valuations \(\valSing\) then we call \(D\) \emph{negatively valid}, denoted
by \(\models_N D\). Otherwise, \(D\) is \emph{negatively falsifiable}.
\end{definition}

We will often omit \(\model\) and \(\valSing\) if they are not necessary for the context.


Note that for both semantics, we have \(\psem{\top}{}{\valSing} = \nsem{\top}{}{\valSing}  =\universe\) and \(\psem{\bot}{}{\valSing} = \nsem{\bot}{}{\valSing} = \emptyset\),
%and the further connectives behave as expected. That is,
However, for a unitary diagram with a single contour and no shaded zones, i.e. \(d = (\{a\}, \emptyset)\), the semantics diverge. In particular, we have \(\psem{d}{}{\valSing} = \val{a}{} \cup \interior{\comp{\val{a}{}}}\) but \(\nsem{d}{}{\valSing} = \universe\).


\begin{tabular}{l|l|l}
  Diagram & Positive&Negative\\
  \hline 
  \unitaryLiteral{a}{.2cm} & \(\val{a}{}\) & \(\interior{\comp{\interior{\comp{\val{a}{}}}}}\)\\
  \unitaryLiteralNeg{a}{.2cm} & \(\interior{\comp{\val{a}{}}}\) & \(\interior{\comp{\val{a}{}}}\)
\end{tabular}


\begin{definition}[Adjacent Zone]
Let \(z = (\zin, \zout)\) be a zone for the contours in
\(\contours\) and \(c \in \contours\). The \emph{zone adjacent to 
\(z\) at \(c\)}, denoted by \(\adj{z}{c}\) is \((\zin \cup \{c\}, \zout \setminus \{c\})\), if \(c \in \zout\)
and \((\zin \setminus \{c\}, \zout \cup \{c\})\) if \(c \in \zin\). 
% \begin{align*}
% \adj{z}{c} &= \left \{
% \begin{array}{ll} 
% (\zin \cup \{c\}, \zout \setminus \{c\}) & \text{ if } c \in \zout\\
% (\zin \setminus \{c\}, \zout \cup \{c\}) & \text{ if } c \in \zin
%  \end{array}  \right.  
% \end{align*}
\end{definition}

Now we can define a way to 
remove contours from a unitary diagram \(d\).
%, such that the conjunction
%of all resulting diagrams is equivalent to \(d\).

\begin{definition}[Reduction]
\label{def:reduction}
Let \(d = (\contours, \zones, \ezones)\) be a unitary Euler diagram and
\(c \in \contours\). The \emph{reduction} of a zone 
\(z = (\zin, \zout)\) is defined by
\(  z \setminus c = (\zin \setminus \{c\}, \zout \setminus \{c\})\).
The \emph{reduction} of \(d\) by \(c\) is defined as \(d \setminus c = (\contours \setminus \{c\}, \zones\setminus c, \ezones \setminus c)\),
where
\begin{align*}
\zones \setminus c & = \{ z \setminus c \mid z \in \zones\}\\
  \ezones \setminus c& = \{z \setminus c \mid z \in \ezones \text{ and } \adj{z}{c} \in \ezones\cup\mzones{d} \} 
\end{align*}
That is, we remove the contour \(c\) from all zones and only shade the reduction of 
a shaded zone \(z\), if  its adjacent zone at \(c\) is shaded or missing. 
\end{definition}

% \begin{definition}[Valuation Restriction]
% Let \(\valSing \colon \vars \to \bool\) a valuation and \(\contours \subseteq \vars\) a
% set of contours. The \emph{restriction of \(\valSing\) to \(\contours\)} 
% is denoted by \(\valSing_{|\contours} \colon \contours \to \bool\).
% We also extend the notion of restrictions to the semantics of diagrams, i.e.,
% \begin{align*}
%   \sem{D}_{|\contours} & = \{ \valSing_{|\contours} \mid \valSing \in \sem{D}\} \enspace.
% \end{align*}
% \end{definition} \slcomment{do we need this definition and the following lemma???}

% \begin{lemma}
% \label{lem:preservation-reduction}
% Let \(d\) be a unitary diagram for the contours \(\contours\) and
% \(d \setminus c\) its reduction by \(c\). Furthermore, let 
% \(\contours_c = \contours \setminus \{c\}\)
% Then \( \sem{d}_{|\contours_c} = \sem{d \setminus c}_{|\contours_c}\). 
% \end{lemma}
% \begin{proof}
% Let \(d\), \(c\) and \(\contours\) be as required and \(\valSing \in \sem{d}\).
% Due to the definition of the semantics of \(d\), this is due to one non-shaded
% zone \(z= (\zin, \zout)\) of \(d\), with \(\valSing \in \sem{z}\).
% %\(\val{a}{} = \ttrue\) for all \(a \in \zin\)
% %and \(\val{a}{} =\ffalse\) for all \(a \in \zout\).  
% Note that 
% for all \(a \in \contours_c\), we have \(\val{a}{} = \val{a}{| \contours_c}\). Hence 
% \(\valSing_{|\contours_c} \in \sem{d \setminus c}_{|\contours_c}\). 

% Conversely, assume that \(\valSing \in \sem{d \setminus c}\) and \(\valSing \not\in\sem{d}\) (otherwise
% there is nothing left to show). This is only possible, if there is a shaded 
% zone \(z = (\zin, \zout) \in \ezones\) of \(d\), such that its reduction \(z^\prime = (\zin \setminus \{c\}, \zout \setminus \{c\})\)
% is not shaded in \(d \setminus c\). Hence, \(\adj{z}{c} \not\in \ezones\) and \(\adj{z}{c} \not \in \mzones{d}\),
% which implies \(\sem{\adj{z}{c}} \in \sem{d}\). Furthermore, for all \(\valSing^\prime \in \sem{\adj{z}{c}}\),
% we have \(\valSing_{|\contours_c} = \valSing^\prime_{|\contours_c}\). Hence \(\valSing_{|\contours_c} \in \sem{d}_{| \contours_c}\).
% \qed
% \end{proof}

 If each
shaded or missing zone in a diagram \(d\) has a shaded or missing adjacent zone,
then the conjunction of the reduction of 
%a diagram
 \(d\) 
by each of its contours preserves the semantic information. That is, 
we can distribute the information contained in \(d\) among simpler diagrams.
% as shown
%in the following lemma. 
\begin{lemma}
\label{lem:sem-intersect-reduction}
Let \(d = (\contours, \zones, \ezones)\), % for the contours \(\contours\), 
where 
for each \(z \in \ezones \cup \mzones{d}\), there is a contour \(\ell \in \contours\) such that 
\(\adj{z}{\ell} \in \ezones \cup \mzones{d}\). Then  %, with \(|\contours| > 1\).
%\begin{align*}
\(  \sem{d} = \bigcap_{c \in \contours} \sem{d \setminus c}\)
%\end{align*} %\slcomment{THIS LEMMA IS WRONG!!!}
%\{\valSing \mid \valSing_{\contours \setminus \{c\}} \in \sem{d \setminus c}_{\contours \setminus \{c\}} \text{ for all } c \in \contours\}
\end{lemma}
\begin{proof}
For each \(c \in \contours\), we have \(\sem{d} \subseteq \sem{d \setminus c}\). % \slcomment{is this true???}
 Hence the direction
from left to right is immediate. Now let \(d = (\contours, \zones, \ezones)\) and 
\(\valSing \) be such that \(\valSing \in \sem{d \setminus c}\) for all
\(c \in \contours\). Hence, for each \(c\),  
there is a \(z_c \in \zones\), such that \(\valSing \in \sem{z_c \setminus c}\).
Now we have to show that in fact there is a \emph{single} zone \(z \in \zones\), 
such that \(\valSing \in \sem{z \setminus c}\) for all \(c\). 
Observe that there are 
%at most
 two zones \(z_\ttrue, z_\ffalse \in \vennzones{d}\) such that
\( \valSing \in \sem{z_\ttrue \setminus c}\) and \( \valSing \in \sem{z_\ffalse \setminus c}\), whose
only difference is that \(c\) is in the in-set of \(z_\ttrue\) and in the out-set of \(z_\ffalse\). 
Now, assume \(\val{c}{} = \ttrue\), hence \(\valSing \in \sem{z_\ttrue}\).
 If \(\valSing \not\in \sem{d}\), this means that \(z_\ttrue \in \ezones \cup \mzones{d}\). By assumption,
 there is a contour \(\ell\) such that \(\adj{z_\ttrue}{\ell} \in \ezones \cup \mzones{d}\).
In the reduction of \(d\) by \(\ell\), this means that \(z_\ttrue\) is either shaded or missing as well,
and hence \(\valSing \not\in \sem{d \setminus \ell}\), which contradicts
the assumption on \(\valSing\). Hence \(\valSing \in \sem{d}\). The case
for \(\val{c}{} = \ffalse\) is similar.
\qed  
\end{proof}

%Note that 
% The precondition in Lemma~\ref{lem:sem-intersect-reduction} corresponds to the
% shading conditions for the rule \emph{Remove Contour} in the work of
%  Stapleton \cite{Stapleton2007} and Howse et al. \cite{Howse2005}. 


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "int-dia-sequent"
%%% End: 

